Possible correlations between gamma-ray burst and its host galaxy offset

We collected the information of 304 gamma-ray bursts (GRBs) from the literature, and analyzed the correlations among the host galaxy offsets (the distance from the site of the GRB to the center of its host galaxy), $T_{\rm 90,i}$ (the duration $T_{\rm 90}$ in rest-frame), $T_{\rm R45,i}$ (the duration $T_{\rm R45}$ in rest-frame), $E_{\rm \gamma,iso}$ (the isotropic equivalent energy), $L_{\rm \gamma,iso}$ ($=E_{\rm \gamma,iso}/T_{\rm 90,i}$, the isotropic equivalent luminosity) and $L_{\rm pk}$ (peak luminosity). We found that $ T_{\rm 90,i}$, $ T_{\rm R45,i}$, $ E_{\rm \gamma,iso}$, $L_{\rm pk}$ have negative correlation with $ {\rm offset}$, which is consistent with origin of short GRBs (SGRBs) and long GRBs (LGRBs). On separate analysis, we found similar results for $\log E_{\rm \gamma,iso}$ - $\log {\rm (offset)}$ and $\log L_{\rm pk}$ - $\log {\rm (offset)}$ relations in case of SGRBs only, while no obvious relation for LGRBs. There is no correlations between offset and $L_{\rm \gamma,iso}$. We also put the special GRB 170817A {and GRB 060218A} on the plots. {The two GRBs both have low luminosity and small offset.} In the $ \log ({\rm offset})- \log T_{\rm 90,i}$ plot, we found GRB 170817A locates in between the two regions of SGRBs and LGRBs and it is the outlier in the $ {\rm offset}-E_{\rm \gamma, iso}$, $ {\rm offset}-L_{\rm \gamma, iso}$ and $ {\rm offset}-L_{\rm pk}$ plots. Together with GRB 060218A being an outlier in all plots, it indicates the speciality of GRBs 170817A and 060218A, and might imply more subgroups of the GRB samples.

==> lpkdata.bak1.tex <==
\begin{landscape}
\begin{table}
\caption{$L_{\rm pk}$ and the related spectral information. The definition of each parameter is shown in Section \ref{sec:samples}.}
\setlength{\tabcolsep}{0pt}
\centering
\small
\begin{tabular}{ccccccc}
\hline
 \multicolumn{1}{c}{GRB}&
  \multicolumn{1}{c}{$L_{\rm pk}$}&
%  \multicolumn{1}{c}{offset}&
  \multicolumn{1}{c}{$-\alpha$}&
  \multicolumn{1}{c}{$-\beta$}&
  \multicolumn{1}{c}{$E_{\rm pk}$}&
  \multicolumn{1}{c}{Model}&
 \multicolumn{1}{c}{ref}
  \\
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm 10^{\rm 52} ~ erg ~ s^{\rm -1}$)}&
 % \multicolumn{1}{c}{($\rm kpc$)}&
   \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm keV$)}&
   \multicolumn{1}{c}{}&
 \multicolumn{1}{c}{} \\
 \hline \\
170817A & $1.6E-5^{\rm +2.5E-5}_{\rm -4E-6}$$\rm{^{d}}$ %& $2.0^{\rm +0.2}_{\rm -0.2}$ 
& ... & ... & ... &  & (1);(2)  \\
130606A & $8^{\rm +2.8}_{\rm -2.1}$$\rm{^{c,d}}$ %& $0.36^{\rm +0.12}_{\rm -0.12}$ 
& $1.140^{\rm +0.091}_{\rm -0.091}$$\rm{^{b}}$ & ... & $294^{\rm +54}_{\rm -30}$$\rm{^{b}}$ & CPL & (3);(4);(4);(4)  \\ 
130427A & $7.1^{\rm +0.3}_{\rm -0.3}$$\rm{^{c,d}}$ %& $4.1^{\rm +0.1}_{\rm -0.1}$ 
& $0.91^{\rm +0.01}_{\rm -0.01}$ & $3.18^{\rm +0.03}_{\rm -0.03}$ & $877.8^{\rm +4.9}_{\rm -4.9}$ & Band & (3);(4);(5);(5);(5)  \\ 
110731A & $8.1^{\rm +1.1}_{\rm -1.1}$$\rm{^{c,d}}$ %& $1.47^{\rm +0.08}_{\rm -0.08}$ 
& $0.82^{\rm +0.03}_{\rm -0.03}$ & $2.32^{\rm +0.03}_{\rm -0.02}$ & $312^{\rm +29}_{\rm -27}$$\rm{^{e}}$ & Band & (3);(4);(6);(6);(6)  \\ 
100816A & $0.984^{\rm +0.022}_{\rm -0.022}$ %& $8.2^{\rm +1.4}_{\rm -1.4}$$\rm{^{b}}$ 
& ... & ... & ... &  & (7);(8)  \\ 
091208B & $2.05^{\rm +0.31}_{\rm -0.41}$ %& 0.79$\rm{^{a}}$ 
& ... & ... & ... &  & (9);(10)   \\ 
091127A & $0.358^{\rm +0.015}_{\rm -0.015}$ %& $1.35^{\rm +0.30}_{\rm -0.30}$ 
& ... & ... & ... &  & (9);(4)  \\ 
090618 & $0.937^{\rm +0.012}_{\rm -0.012}$ %& $4.5^{\rm +0.3}_{\rm -0.3}$ 
& ... & ... & ... &  & (7);(4)   \\ 
090426 & $2.90^{\rm +0.78}_{\rm -0.63}$$\rm{^{c,d}}$ %& $0.49^{\rm +0.25}_{\rm -0.25}$ 
& $1.93^{\rm +0.13}_{\rm -0.13}$$\rm{^{b}}$ & ... & ... & SPL & (3);(4);(4) \\ 
090424A & $1.680^{\rm +0.029}_{\rm -0.029}$ %& $2.62^{\rm +0.24}_{\rm -0.24}$ 
& ... & ... & ... &  & (7);(4)  \\ 
090418A & $1.18^{\rm +0.19}_{\rm -0.34}$ % & 0.74$\rm{^{a}}$ 
& ... & ... & ... &  & (9);(10) \\ 
090205A & $1.30^{\rm +1.4}_{\rm -0.94}$$\rm{^{c,d}}$ %& $2.7^{\rm +2.0}_{\rm -2.0}$ 
& $1.0^{\rm +0.6}_{\rm -1.2}$$\rm{^{b}}$ & ... & $33^{\rm +19}_{\rm -19}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11)  \\ 
090102A & $5.83^{\rm +0.84}_{\rm -0.82}$ %& $0.78^{\rm +0.52}_{\rm -0.52}$ 
& ... & ... & ... &  & (9);(4) \\ 
081221A & $11.8^{\rm +0.2}_{\rm -0.2}$ %& $3.3^{\rm +0.6}_{\rm -0.6}$ 
& ... & ... & ... &  & (7);(4) \\ 
081121A & $5.37^{\rm +0.74}_{\rm -0.74}$ %& $2^{\rm +1}_{\rm -1}$ 
& ... & ... & ... &  & (7);(4) \\ 
081008A & $0.55^{\rm +0.14}_{\rm -0.14}$$\rm{^{c,d}}$ %& $14.3^{\rm +0.2}_{\rm -0.2}$ 
& $1.010^{\rm +0.073}_{\rm -0.073}$$\rm{^{b}}$ & $2.09^{\rm +0.13}_{\rm -0.13}$$\rm{^{b}}$ & $166^{\rm +22}_{\rm -22}$$\rm{^{b}}$ & Band & (3);(4);(12);(12);(12) \\ 
081007A & $0.034^{\rm +0.016}_{\rm -0.014}$$\rm{^{c,d}}$ %& $0.71^{\rm +0.18}_{\rm -0.18}$ 
& $1.40^{\rm +0.36}_{\rm -0.6}$$\rm{^{b}}$ & ... & $27.0^{\rm +6.7}_{\rm -9.7}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11)  \\ 
080928 & $0.474^{\rm +0.18}_{\rm -0.084}$$\rm{^{c,d}}$ %& $14.8^{\rm +0.3}_{\rm -0.3}$ 
& $1.70^{\rm +0.06}_{\rm -0.06}$$\rm{^{b}}$ & ... & $74^{\rm +147}_{\rm -16}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11) \\ 
080916A & $0.108^{\rm +0.005}_{\rm -0.005}$ %& 0.14$\rm{^{a}}$ 
& ... & ... & ... &  & (7);(10) \\ 
080805A & $0.211^{\rm +0.11}_{\rm -0.051}$$\rm{^{c,d}}$ %& $4.0^{\rm +0.4}_{\rm -0.4}$ 
& $1.540^{\rm +0.054}_{\rm -0.054}$$\rm{^{b}}$ & ... & $300^{\rm +333}_{\rm -115}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11) \\ 
080707A & $0.221^{\rm +0.076}_{\rm -0.073}$$\rm{^{c,d}}$ %& $0.76^{\rm +0.46}_{\rm -0.46}$ 
& $1.78^{\rm +0.17}_{\rm -0.17}$ & ... & ... & SPL & (3);(4);(13)  \\
080607A & $129^{\rm +26}_{\rm -26}$ %& $5.4^{\rm +1.9}_{\rm -1.9}$ 
& ... & ... & ... &  & (9);(4)  \\ 
080605A & $9.82^{\rm +0.18}_{\rm -0.18}$ %& $0.70^{\rm +0.27}_{\rm -0.27}$ 
& ... & ... & ... &  & (7);(4)  \\ 
080430 & $0.103^{\rm +0.13}_{\rm -0.007}$ %& $0.81^{\rm +0.37}_{\rm -0.37}$ 
& ... & ... & ... &  & (14);(4)  \\ 
080319C & $6.04^{\rm +8}_{\rm -0.42}$ %& $7.4^{\rm +0.4}_{\rm -0.4}$ 
& ... & ... & ... &  & (14);(4)  \\   
      \hline
\end{tabular}
\\
\begin{flushleft} 
$\rm{^{a}}$ - The errors are imputed by MICE algorithm.\\
$\rm{^{b}}$ - The errors in the original papers are in 90$\%$ confidence level, we changed the errors to 1 $\sigma$ confidence level by multiplying 0.995/1.645. \\
$\rm{^{c}}$ - The values are calculated using the spectral values in order to change the energy band. \\
$\rm{^{d}}$ - We changed the values into logarithm or from logarithm into the normal form. \\
$\rm{^{e}}$ - The values are calculated using $\alpha$ and break energy $E_{0}$. \\
$\rm{^{f}}$ - The peak luminosity of GRB 170817A is derived from 50 $\rm ms$ time resolution light curve. \\
\end{flushleft}
\label{tab:lpk}
\end{table}
\end{landscape}


\begin{landscape}
\begin{table}
\caption{Continued from previous page}
\setlength{\tabcolsep}{0pt}
\centering
\small
\begin{tabular}{cccccccc}
\hline
 \multicolumn{1}{c}{GRB}&
  \multicolumn{1}{c}{$L_{\rm pk}$}&
  \multicolumn{1}{c}{$-\alpha$}&
  \multicolumn{1}{c}{$-\beta$}&
  \multicolumn{1}{c}{$E_{\rm pk}$}&
  \multicolumn{1}{c}{Model}&
 \multicolumn{1}{c}{ref}
  \\
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm 10^{\rm 52} ~ erg ~ s^{\rm -1}$)}&
  \multicolumn{1}{c}{($\rm kpc$)}&
   \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm keV$)}&
   \multicolumn{1}{c}{}&
 \multicolumn{1}{c}{} \\
 \hline \\
 080319B & $7.39^{\rm +0.71}_{\rm -0.71}$ & ... & ... & ... &  & (9);(4)  \\ 
080207A & $0.61^{\rm +0.11}_{\rm -0.11}$ & ... & ... & ... &  & (7);(4)  \\ 
071227A & $0.0334^{\rm +0.0049}_{\rm -0.0049}$ & ... & ... & ... &  & (15);(4)   \\ 
071122 & $0.035^{\rm +0.06}_{\rm -0.026}$$\rm{^{c,d}}$  & $1.60^{\rm +0.24}_{\rm -0.24}$$\rm{^{b}}$ & ... & $111^{\rm +318}_{\rm -41}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11)   \\ 
 071112C & $4.0^{\rm +1.1}_{\rm -1.1}$$\rm{^{c,d}}$  & $1.090^{\rm +0.042}_{\rm -0.042}$$\rm{^{b}}$ & ... & ... & SPL & (3);(4);(16) \\
071010A & $1.97^{\rm +0.9}_{\rm -0.78}$$\rm{^{c,d}}$  & ... & ... & SPL & (3);(10);(4) \\
071010B & $0.605^{\rm +0.014}_{\rm -0.014}$ & ... & ... & ... &  & (7);(4) \\
070802A & $0.24^{\rm +0.2}_{\rm -0.14}$$\rm{^{c,d}}$  & $1.80^{\rm +0.18}_{\rm -0.18}$$\rm{^{b}}$ & ... & $55^{\rm +161}_{\rm -21}$$\rm{^{b}}$ & CPL & (3);(4);(11);(11)  \\
 070724A & $0.0158^{\rm +0.0034}_{\rm -0.0014}$  & ... & ... & ... &  & (15);(4)  \\ 
070714B & $1.45^{\rm +0.17}_{\rm -0.38}$ & ... & ... & ... &  & (9);(4)  \\ 
070508 & $2.374^{\rm +0.037}_{\rm -0.037}$  & ... & ... & ... &  & (7);(4)  \\ 
070429B & $0.246^{\rm +0.038}_{\rm -0.038}$  & ... & ... & ... &  & (15);(17)  \\
070318A & $0.073^{\rm +0.048}_{\rm -0.015}$$\rm{^{c,d}}$ & $1.410^{\rm +0.048}_{\rm -0.048}$$\rm{^{b}}$ & ... & $196^{\rm +269}_{\rm -47}$$\rm{^{b}}$ & CPL & (3);(4);(18);(18) \\ 
070306A & $0.867^{\rm +1.4}_{\rm -0.027}$  & ... & ... & ... &  & (14);(4)  \\ 
061217 & $0.108^{\rm +0.018}_{\rm -0.018}$ & ... & ... & ... &  & (15);(19) \\ 
061210A & $0.215^{\rm +0.014}_{\rm -0.014}$  & ... & ... & ... &  & (15);(19) \\ 
061110B & $0.59^{\rm +0.94}_{\rm -0.38}$$\rm{^{c,d}}$  & $0.70^{\rm +0.12}_{\rm -0.12}$$\rm{^{b}}$ & ... & $550^{\rm +593}_{\rm -151}$$\rm{^{b}}$ & CPL & (3);(4);(18);(18)  \\ 
061110A & $0.0170^{\rm +0.011}_{\rm -0.0051}$$\rm{^{c,d}}$ & $1.60^{\rm +0.06}_{\rm -0.06}$$\rm{^{b}}$ & ... & $106^{\rm +181}_{\rm -24}$$\rm{^{b}}$ & CPL & (3);(4);(18);(18)   \\ 
061007A & $14.3^{\rm +2.3}_{\rm -1.8}$ & ... & ... & ... &  & (9);(10)  \\ 
061006A & $0.2460^{\rm +0.012}_{\rm -0.0077}$  & ... & ... & ... &  & (15);(4)  \\ 
060912A & $1.076^{\rm +0.16}_{\rm -0.095}$$\rm{^{c}}$ & $5.2^{\rm +1.2}_{\rm -1.2}$  & ... & $200^{\rm +339}_{\rm -67}$$\rm{^{b}}$ & CPL & (20);(4);(18);(18) \\ 
060801A & $0.476^{\rm +0.062}_{\rm -0.016}$  & ... & ... & ... &  & (15);(17) \\ 
060729A & $0.0196^{\rm +0.0085}_{\rm -0.0041}$$\rm{^{c,d}}$  & $1.80^{\rm +0.06}_{\rm -0.06}$$\rm{^{b}}$ & ... & $67^{\rm +139}_{\rm -15}$$\rm{^{b}}$ & CPL & (3);(4);(18);(18) \\ 
060719A & $0.54^{\rm +0.16}_{\rm -0.15}$$\rm{^{c,d}}$  & $1.90^{\rm +0.06}_{\rm -0.06}$$\rm{^{b}}$ & ... & $55^{\rm +31}_{\rm -31}$$\rm{^{b}}$ & CPL & (3);(4);(18);(18)  \\ 
060614A & $0.00808^{\rm +0.0013}_{\rm -0.00094}$ & ... & ... & ... &  & (9);(4)  \\ 
060605A & $0.91^{\rm +0.13}_{\rm -0.13}$ & ... & ... & ... &  & (21);(4) \\ 
060602A & $0.061^{\rm +0.025}_{\rm -0.008}$  & ... & ... & ... &  & (15);(10)  \\ 
060522 & $2.33^{\rm +0.78}_{\rm -0.81}$ & ... & ... & ... &  & (9);(4)   \\ 
060502B & $0.0065^{\rm +9E-4}_{\rm -9E-4}$ & ... & ... & ... &  & (15);(19)  \\
060418A & $1.96^{\rm +0.43}_{\rm -0.13}$  & ... & ... & ... &  & (14);(4)   \\ 
060218A & $4.3E-6^{\rm +1.5E-6}_{\rm -1.7E-6}$ & ... & ... & ... &  & (9);(4)  \\ 
060206A & $7.18^{\rm +0.27}_{\rm -0.27}$  & ... & ... & ... &  & (7);(4)  \\ 
     \hline
\end{tabular}
\\
%\label{tab:sample}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\caption{Continued from previous page}
\setlength{\tabcolsep}{0pt}
\centering
\small
\begin{tabular}{cccccccc}
\hline
 \multicolumn{1}{c}{GRB}&
  \multicolumn{1}{c}{$L_{\rm pk}$}&
  \multicolumn{1}{c}{$-\alpha$}&
  \multicolumn{1}{c}{$-\beta$}&
  \multicolumn{1}{c}{$E_{\rm pk}$}&
  \multicolumn{1}{c}{Model}&
 \multicolumn{1}{c}{ref}
  \\
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm 10^{\rm 52} ~ erg ~ s^{\rm -1}$)}&
  \multicolumn{1}{c}{($\rm kpc$)}&
   \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm keV$)}&
   \multicolumn{1}{c}{}&
 \multicolumn{1}{c}{} \\
 \hline \\
 060124A & $10.2^{\rm +3.1}_{\rm -2.9}$   & ... & ... & ... &  & (9);(4)   \\ 
060121A & $24.5^{\rm +1.6}_{\rm -1.6}$  & ... & ... & ... &  & (15);(4)   \\ 
060115A & $1.55^{\rm +0.13}_{\rm -0.13}$  & ... & ... & ... &  & (7);(4)   \\ 
051221A & $0.258^{\rm +0.009}_{\rm -0.009}$  & ... & ... & ... &  & (15);(4)  \\ 
051022A & $3.12^{\rm +0.41}_{\rm -0.41}$  & ... & ... & ... &  & (9);(4)  \\ 
051016B & $0.065^{\rm +0.048}_{\rm -0.038}$   & ... & ... & ... &  & (9);(4) \\ 
050904A & $8.5^{\rm +2.3}_{\rm -2.4}$  & ... & ... & ... &  & (9);(4)  \\ 
050826A & $0.0033^{\rm +0.0032}_{\rm -8E-4}$  & ... & ... & ... &  & (15);(4)  \\ 
 050824A & $0.18^{\rm +0.19}_{\rm -0.17}$$\rm{^{c,d}}$   & $2.76^{\rm +0.23}_{\rm -0.23}$$\rm{^{b}}$ & ... & ... & SPL & (3);(4);(4)  \\ 
050820A & $3.22^{\rm +0.3}_{\rm -0.45}$   & ... & ... & ... &  & (9);(4)  \\ 
050813 & $0.04^{\rm +0.02}_{\rm -0.02}$  & ... & ... & ... &  & (15);(17)  \\ 
050724A & $0.0099^{\rm +0.0023}_{\rm -0.001}$  & ... & ... & ... &  & (15);(4)  \\ 
050709A & $0.0540^{\rm +0.0067}_{\rm -0.0069}$  & ... & ... & ... &  & (15);(4)  \\ 
050525A & $1.159^{\rm +0.016}_{\rm -0.016}$  & ... & ... & ... &  & (7);(4)  \\ 
050509B & $7E-4^{\rm +0.001}_{\rm -5E-4}$  & ... & ... & ... &  & (15);(4)  \\ 
050416A & $0.087^{\rm +0.019}_{\rm -0.015}$  & ... & ... & ... &  & (9);(4)  \\ 
 050401A & $12.0^{\rm +2.3}_{\rm -2.6}$   & ... & ... & ... &  & (9);(4)  \\ 
050315 & $0.88^{\rm +0.33}_{\rm -0.31}$   & ... & ... & ... &  & (9);(4)  \\ 
041006A & $0.531^{\rm +0.022}_{\rm -0.022}$   & ... & ... & ... &  & (9);(4)  \\ 
040924A & $0.86^{\rm +0.09}_{\rm -0.09}$  & ... & ... & ... &  & (9);(4)  \\ 
030429A & $0.75^{\rm +0.19}_{\rm -0.22}$   & ... & ... & ... &  & (9);(4)  \\ 
030323A & $1.14^{\rm +0.61}_{\rm -0.51}$  & ... & ... & ... &  & (9);(4)  \\ 
021004A & $0.91^{\rm +0.19}_{\rm -0.19}$   & ... & ... & ... &  & (9);(4)  \\ 
010921A & $0.13^{\rm +0.01}_{\rm -0.01}$   & ... & ... & ... &  & (21);(4)   \\ 
010222A & $28.7^{\rm +1.3}_{\rm -1.2}$  & ... & ... & ... &  & (9);(4)  \\ 
000210A & $7.0^{\rm +2.8}_{\rm -1.8}$   & ... & ... & ... &  & (9);(4) \\ 
991208A & $4.68^{\rm +1.2}_{\rm -0.83}$   & ... & ... & ... &  & (9);(4)  \\ 
     \hline
\end{tabular}
\\
\end{table}
\end{landscape}


\begin{table}
\caption{Continued from previous page}
\setlength{\tabcolsep}{0pt}
\centering
\small
\begin{tabular}{cccccccc}
\hline
 \multicolumn{1}{c}{GRB}&
  \multicolumn{1}{c}{$L_{\rm pk}$}&
  \multicolumn{1}{c}{$-\alpha$}&
  \multicolumn{1}{c}{$-\beta$}&
  \multicolumn{1}{c}{$E_{\rm pk}$}&
  \multicolumn{1}{c}{Model}&
 \multicolumn{1}{c}{ref}
  \\
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm 10^{\rm 52} ~ erg ~ s^{\rm -1}$)}&
  \multicolumn{1}{c}{($\rm kpc$)}&
   \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c}{($\rm keV$)}&
   \multicolumn{1}{c}{}&
 \multicolumn{1}{c}{} \\
 \hline \\
990705A & $2.21^{\rm +0.19}_{\rm -0.17}$ & ... & ... & ... &  & (9);(4)   \\ 
990510A & $5.2^{\rm +1.1}_{\rm -1.4}$   & ... & ... & ... &  & (9);(4)  \\
990123A & $27.5^{\rm +1.2}_{\rm -1.2}$   & ... & ... & ... &  & (9);(4)   \\
980703A & $1.20^{\rm +0.13}_{\rm -0.23}$  & ... & ... & ... &  & (9);(4)   \\ 
980613A & $0.193^{\rm +0.068}_{\rm -0.057}$   & ... & ... & ... &  & (9);(4)  \\ 
971214B & $9.5^{\rm +5.3}_{\rm -4}$   & ... & ... & ... &  & (9);(22)  \\ 
970508A & $0.164^{\rm +0.021}_{\rm -0.021}$  & ... & ... & ... &  & (9);(22)  \\ 
970228A & $1.54^{\rm +0.21}_{\rm -0.12}$   & ... & ... & ... &  & (9);(4) \\ 
     \hline
\end{tabular}
\\
\label{tab:lpklast}
\end{table}


References.                                  
(1) \citet{Zhang5851};                
(2) \citet{AbbottA2017};        
(3) \citet{Deng2016};           
(4) \citet{Li2016ApJS};                 
(5) \citet{Goldstein2016};                
(6) \citet{Ackermann2013};                      
(7) \citet{Lin2016};
(8) \citet{Kopac2012};
(9) \citet{Yonetoku2010};
(10) \citet{Lyman2017};
(11) \citet{Butler2010};
(12) \citet{Heussaff2013};
(13) \citet{Krimm2009};
(14) \citet{Ukwatta2010};
(15) \citet{Zhang2009};
(16) \citet{Nava2012};
(17) \citet{Tunnicliffe2014};
(18) \citet{Butler2007};
(19) \citet{Cui2012};
(20) \citet{Rizzuto2007};
(21) \citet{Rossi2008};
(22) \citet{Bloom2002}
